Graph Representation Learning via Multi-task Knowledge Distillation

Machine learning on graph structured data has attracted much research interest due to its ubiquity in real world data. However, how to efficiently represent graph data in a general way is still an open problem. Traditional methods use handcraft graph features in a tabular form but suffer from the defects of domain expertise requirement and information loss. Graph representation learning overcomes these defects by automatically learning the continuous representations from graph structures, but they require abundant training labels, which are often hard to fulfill for graph-level prediction problems. In this work, we demonstrate that, if available, the domain expertise used for designing handcraft graph features can improve the graph-level representation learning when training labels are scarce. Specifically, we proposed a multi-task knowledge distillation method. By incorporating network-theory-based graph metrics as auxiliary tasks, we show on both synthetic and real datasets that the proposed multi-task learning method can improve the prediction performance of the original learning task, especially when the training data size is small.

==> related.tex <==
\section{Related Work}
\subsection{Graph Representation Learning}
Representation learning methods attempt to represent discrete objects as vectors in a continuous space (a.k.a., embedding) so that similar objects have similar embedding vectors. In the context of graph, the object to be represented can be either a node \cite{perozzi2014deepwalk, grover2016node2vec, tang2015line}, a subgraph of a graph \cite{narayanan2016subgraph2vec, yanardag2015deep, li2017deepcas}, or an entire graph \cite{atwood2016diffusion, li2016deepgraph, niepert2016learning}. Most of these works are inspired by the huge success of representation learning and deep learning applied to various domains such as text \cite{bengio2003neural} and image \cite{krizhevsky2012imagenet}. For node-level and subgraph-level representation learning, the models usually assume there is a giant graph in which the nodes and subgraphs reside in. In such cases, an analogy can be made between the nodes in graphs and the words in natural language, where both scenarios have a ``corpus'' shared by all data instances. For example, DeepWalk \cite{perozzi2014deepwalk} uses fixed-length random walk paths to stimulate the ``context'' of a node so that node representations can be learned using the same unsupervised method of learning word representations \cite{mikolov2013efficient}. In the case of graph-level representation learning, however, there is no such a shared ``corpus'' so the unsupervised methods in natural language processing are no longer applicable. Moreover, the labels of entire graphs are usually fewer comparing to those of nodes and subgraphs. In this paper, we focus on the problem of graph-level representation learning and tackle the scenario where labels are too few for the supervised learning method to be effective for the deep neural network models.

\subsection{Graph-level Prediction}
A graph-level prediction problem is a supervised learning problem where the input is an entire graph and the output is a label associated to this graph. The main difference between a graph-level prediction problem and a subgraph-level prediction problem is that the input graphs of a graph-level problem are independent of each other while the input graphs of a subgraph-level problem are assumed resides in a same giant graph. The methods used in the graph-level prediction problems can be categorized into 3 groups in terms of how they model the input graph. The first group of methods \cite{kupavskii2012prediction, szabo2010predicting} calculate graph features out of the input graph and then feed the features into a traditional machine learning models designed for vector inputs. The second group of methods \cite{kashima2004kernels, bai2015quantum, shervashidze2009efficient, shervashidze2011weisfeiler, yanardag2015deep} introduce kernels for graphs and then apply kernel methods on graph kernels. Graph kernels provide an indirect way to model graph representations. The third group of methods \cite{atwood2016diffusion, li2016deepgraph, niepert2016learning} are graph representation learning methods mentioned above. This work belongs to the third group of methods but we also compare with the state-of-the-art graph kernel methods on real benchmark graph prediction datasets. 

\subsection{Multi-task Learning}
By learning multiple tasks at the same time, multi-task models can learn commonalities across tasks. This can result in both improved statistical efficiency and model quality for each task. The multi-task learning model framework proposed by Caruana \cite{caruana1998multitask} is the most widely used structure used in multi-task neural network models. As shown as the ``Multi-task Learning Framework'' block in Figure \ref{fig:model}, this framework consists of two main parts: a bottom part follows the input data and is shared by all the tasks; a top part follows the shared bottom part and contains several parallel pieces sub-network with each piece leads to an output for an individual task. Recently, there are many successful applications of this framework in the domain of image \cite{girshick2015fast, ren2015faster} and natural language \cite{collobert2008unified}. In this paper, we adopt the same multi-task neural network model structure but introduce a novel paradigm of multi-task learning in graph prediction problems.

\subsection{Network Theory}
There are two active research directions related to this work: network metrics and random graph models. 

Researchers have developed many measures and metrics in network theory to quantify network structures, which are the foundations of the subsequent network analysis problems \cite{newman2010networks}. Previous works \cite{kupavskii2012prediction, szabo2010predicting} have shown that such network metrics also help with predictions on graph data when serving as features in a machine learning model. Such network metrics surely contain knowledge that represent some properties of a network and it is desirable to distill such knowledge into the graph representation learned by deep neural network models. In this paper, we incorporate network metrics as auxiliary tasks in a multi-task neural network model so that the internal graph representations learned by the model will also try to reflect some key properties in network theory. 

In network theory, random graph models are widely studied to both understand consequences of certain network properties and mimic the real world networks for simulation purposes \cite{newman2010networks}. In this paper, we also use random graph models in two ways similar with the aforementioned purposes. First, we generate synthetic data using three common random graph models and conduct control experiments on top of them to verify the proposed method. Second, we generate random graphs that mimic the real dataset and use the random graphs as data augmentation for the real dataset. 

\subsection{Knowledge Distillation}
Hinton et al. \cite{hinton2015distilling} suggested an abstract view of the knowledge, that is learned in a machine learning model, as the mapping from inputs to outputs. They also showed in \cite{hinton2015distilling} that a neural network model is able to learn from such mappings given as input-output pairs. Inspired by the concept that knowledge is not stored in the learned model parameters but in the input-output mapping, we come up with the method that use network metrics as auxiliary tasks in the graph representation learning. 
